SemEval-2024 Task 9: BRAINTEASER: A Novel Task Defying Common Sense

While vertical thinking relies on logical and commonsense reasoning, lateral thinking requires systems to defy commonsense associations and overwrite them through unconventional thinking. Lateral thinking has been shown to be challenging for current models but has received little attention. A recent benchmark, BRAINTEASER, aims to evaluate current models' lateral thinking ability in a zero-shot setting. In this paper, we split the original benchmark to also support fine-tuning setting and present SemEval Task 9: BRAIN-TEASER(S), the first task at this competition designed to test the system's reasoning and lateral thinking ability. As a popular task, BRAINTEASER(S)'s two subtasks receive 483 team submissions from 182 participants during the competition. This paper provides a fine-grained system analysis of the competition results, together with a reflection on what this means for the ability of the systems to reason laterally. We hope that the BRAINTEASER(S) subtasks and findings in this paper can stimulate future work on lateral thinking and robust reasoning by computational models.

==> sections/related_work.tex <==
\section{Related Work}
\noindent \textbf{Commonsense reasoning} has been a long-standing goal of NLP and AI, with recent work geared towards scalable evaluation~\cite{talmor-etal-2019-commonsenseqa,sap-etal-2019-social}, generalizable reasoning~\cite{ma-etal-2021-exploring,lourie2021unicorn}, and large-scale knowledge sources~\cite{speer2017conceptnet,Hwang2021COMETATOMIC2O}. \textsc{BrainTeaser} incorporates common sense in a novel way: commonsense knowledge serves as a default reasoning distractor, making it difficult for machines to overwrite it.

\noindent \textbf{Adversarial robustness} investigates whether AI can generalize well to novel tasks and situations, often designed in a way that may exhibit a particular weakness~\cite{jia-liang-2017-adversarial,zellers-etal-2019-hellaswag,nie-etal-2020-adversarial,goldberg2023two}. \textsc{BrainTeaser}'s unseen teasers should be attractive for researchers working on adversarial robustness.

\noindent \textbf{Computational creativity} research has focused on evaluating and building systems for pun detection~\cite{zou-lu-2019-joint}, riddles~\cite{lin-etal-2021-riddlesense}, and humor~\cite{meaney-etal-2021-semeval}. \textsc{BrainTeaser} complements these tasks that require unconventional thinking with novel subtasks on reverse thinking and word games, which we expect to be inspiring for this community.
